Comparison and Application of non-Conforming Mesh Models for Flow in Fractured Porous Media using dual {L}agrange multipliers

Geological settings with reservoir characteristics include fractures with different material and geometrical properties. Hence, numerical simulations in applied geophysics demands for computational frameworks which efficiently allow to integrate various fracture geometries in a porous medium matrix. This study presents a modeling approach for single-phase flow in fractured porous media and its application to different types of non-conforming mesh models. We propose a combination of the Lagrange multiplier method with variational transfer to allow for complex non-conforming geometries as well as hybrid- and equi-dimensional models and discretizations of flow through fractured porous media. The variational transfer is based on the $L^2$-projection and enables an accurate and highly efficient parallel projection of fields between non-conforming meshes (e.g.,\ between fracture and porous matrix domain). We present the different techniques as a unified mathematical framework with a practical perspective. By means of numerical examples we discuss both, performance and applicability of the particular strategies. Comparisons of finite element simulation results to widely adopted 2D benchmark cases show good agreement and the dual Lagrange multiplier spaces show good performance. In an extension to 3D fracture networks, we first provide complementary results to a recently developed benchmark case, before we explore a complex scenario which leverages the different types of fracture meshes. Complex and highly conductive fracture networks are found more suitable in combination with embedded hybrid-dimensional fractures. However, thick and blocking fractures are better approximated by equi-dimensional embedded fractures and the equi-dimensional mortar method, respectively.

==> CompFrac ArXiv/tables/results_2DHydro.tex <==
\scriptsize
\centering
\begin{tabular}{llrrll}
\toprule\bfseries \# uniform ref & \bfseries \#-elem & \bfseries \# nodes. & \bfseries err$_m$ \\\midrule
1 & 272.    & 159       & 0.000512563\\
2 & 1088   & 589      & 8.50172e-05\\
3 & 4352   & 2265     & 1.66138e-05\\
4 & 17408  &  8881   &  4.06608e-06\\
5 & 69632  & 35169   & 1.92418e-06\\
6 & 278528 & 139969 &1.30185e-06\\
\bottomrule
\end{tabular}

\vspace{1cm}



==> CompFrac ArXiv/tables/results_2DHydroCoinAMR.tex <==
\scriptsize
\centering
\begin{tabular}{llrrllllll}
\toprule\bfseries Method & \bfseries \#-matr. & \bfseries \#-frac. & \bfseries d.o.f. & \bfseries nnz/size$^2$ & \bfseries $\| \cdot \|_2$-cond. & \bfseries err$_m$ &\bfseries \# AR & \bfseries err$_g$ \\\midrule
Embedded-ED & \,611 triangles & 3 480 &  352 & 2.0e-2 & 1.5e10 & 8.9e-5 & 0 (2) & -\\
Embedded-ED  & 1 544 triangles&  3 480 & 874 & 7.8e-3 & 5.3e10 & 1.6e-5 & 1 (2) & 5\\
Embedded-ED  & 2 378 triangles&  3 480 & 1354 & 4.5e-3 &  8.1e10 & 7.2e-5 & 2 (2) & 5\\
Embedded-ED  & 7 913 triangles&  3 480 &  4371 &  1.6e-3 & 3.5e11 & 2.9e-6 & 4 (2) & 1\\
Embedded-ED & 9 147 triangles&  3 480& 4991 & 1.5e-3 & 2.8e11 & 2.0e-6 & 4 (4) & 1\\
Embedded-ED & 21 599 triangles & 3 480 & 11658 & 1.02e-3 & 1.06e12 & 1.4e-6 & 4 (6) & 1\\
\hline
Mortar-ED & 2 127 triangles & 202 & 1375 & 5.9e-3 & 3.7e11 & 2.1e-4 & 1 (1) & 5\\
Mortar-ED & 8004 triangles & 332 & 2791 & 1.1e-3 & 1.9e12 & 1.9e-4 & 2 (2) & 5\\
Mortar-ED & 19 515 triangles & 442 & 10 600 & 7.1e-4 & 1.2e12 & 1.9e-4 & 3 (2) & 5\\
Mortar-ED&  28 692 triangles  & 457 & 15 284 &  4.8e-4 & 1.7e12 & 1.9e-4 & 4 (2) & 5\\
\bottomrule
\end{tabular}


==> CompFrac ArXiv/tables/results_2DHydroCoinUR.tex <==
\scriptsize
\centering
\begin{tabular}{llrrllll}
\toprule\bfseries Method & \bfseries \#-matr. & \bfseries \#-frac. & \bfseries d.o.f. & \bfseries nnz/size$^2$ & \bfseries $\| \cdot \|_2$-cond. & \bfseries err$_m$ & \#\textbf{UR} \\\midrule
Embedded-ED & 272 triangles & 3 480 &  159 & 4.3e-2 & 2.9e9 & 5.1e-4& 1\\
Embedded-ED & 1 088 triangles&  3 480 & 589 & 1.2e-2 & 1.1e10 & 8.5e-5&2\\
Embedded-ED  & 4 352 triangles&  3 480 & 2 265 & 3.1e-2 &  4.3e10 & 1.7e-5&3\\
Embedded-ED & 17 408 triangles&  3 480 &  8 881 &  8.1e-4 & 1.8e11 & 4.0e-6& 4\\
Embedded-ED & 69 632 triangles&  3 480& 35 169 & 2.1e-4 & 6.8e11 & 1.9e-6 & 5\\
Embedded-ED & 278 528 triangles & 3 480 & 139 969 & 5.5e-5 & 2.7e12 & 1.3e-6 & 6\\
\hline
Mortar-ED & 1 116 triangles & 220 & 246 &  9.7e-3& 3.6e6 &2.1e-4 & 1\\
Mortar-ED & 4 464 triangles & 880 & 2 973 & 2.5e-3 & 7.6e6 & 1.9e-4 & 2 \\
Mortar-ED & 17 856 triangles & 3520 & 11\,285 &  6.4e-4 & 2.7e7 & 2.0e-4 & 3\\
Mortar-ED &  71 424 triangles & 14 080 & 43 941 &  1.7e-4 & 1.1e8 & 2.0e-4 & 4\\
\bottomrule
\end{tabular}


==> CompFrac ArXiv/tables/results_2DReal.tex <==
\scriptsize
\centering
\begin{tabular}{llrrllll}
\toprule\bfseries Method & \bfseries \#-matr. & \bfseries \#-frac. & \bfseries d.o.f. & \bfseries nnz/size$^2$ & \bfseries $\| \cdot \|_2$-cond.\\\midrule
Embedded-ED & 1405 quads & 199 996 & 1487 &  1.9e-4 & 2.0e15\\
Embedded-ED & 39 085 quads & 199 996 & 41\;773 &  2.3e-4 & 2.2e17\\
Embedded-ED & 94 513 quads & 199 996 & 102\;486 & 9.1e-5 & 5.8e17\\
\hline
Embedded-HD & 4200 quads & 1024 & 4331 & 3.8e-3 & 1.3e16\\
Embedded-HD & 67 200 quads & 4096 & 67\,721 & 1.6e-4 & 2.1e17\\

\bottomrule
\end{tabular}

==> CompFrac ArXiv/tables/results_2DRegular.tex <==
\scriptsize
\centering
\begin{tabular}{llrrllll}
\toprule\bfseries Method & \bfseries \#-matr. & \bfseries \#-frac. & \bfseries d.o.f. & \bfseries nnz/size$^2$ & \bfseries $\| \cdot \|_2$-cond. & \bfseries err$_m$ \\\midrule
Embedded-ED & 10 656 triangles & 8648 & 5853 & 1.3e-3 & 3.7e6 & 3.3e-5\\
Embedded-ED & 47 142 triangles& 8648 & 25\,992 & 2.8e-4 & 1.8e8 & 1.9e-6\\
Embedded-ED & 96 762 triangles& 8648 & 53\,379 & 1.4e-4 &  1.2e9 & 2.8e-7\\
\hline
Mortar-ED & 12 791 triangles& 34 592 & 32\,935 &  2.3e-4 & 5.2e10 & 6.4e-8\\
Mortar-ED & 36 331 triangles& 34 592 & 45\,172 & 1.7e-4 & 8.8e10 & 2.8e-8\\
\hline
Mortar-ED (blocking) & 922 triangles& 34 592 & 26\,520 & 2.7e-4 & 9.4e7 & 3.3e-8\\
\hline
Embedded-HD & 1089 quads& 112 & 1156 & 9.7e-3 & 3.0e4 & 9.7e-3\\
Embedded-HD & 16 641 quads & 448 & 16\,900 & 5.6e-4 & 1.6e6 & 2.5e-3\\
Embedded-HD & 66 049 quads & 896 & 66\,564 &  1.4e-4 & 1.3e7 & 1.3e-3\\

\bottomrule
\end{tabular}


==> CompFrac ArXiv/tables/table_methods.tex <==
\scriptsize
\centering
\begin{tabular}{llrrllll}
\toprule\bfseries Method & \bfseries \#-matr. & \bfseries \#-frac. & \bfseries d.o.f. & \bfseries err$_m$ & \bfseries err$_f$ & \bfseries nnz/size$^2$ & \bfseries $\| \cdot \|_2$-cond.\\\midrule
Embedded equi-dimension model$^2$ & 1496 quads & 78 & 1733.0 & 1.2e-2 & 7.6e-3 & 5.2e-3 & 5.4e12\\
Embedded hybrid-dimensional model$^2$ - dual-Lagr.-Mult. & 1496 quads & 78 & 1575.0 & 1.2e-2 & 7.6e-3 & 6.6e-3 & 7.9e10\\
Mortar equi-dimesional model$^2$ - p0-Lagr.-Mult. & 1496 quads & 78 & 1732.0 & 1.2e-2 & 7.8e-3 & 5.0e-3 & 2.8e12\\
\bottomrule
\end{tabular}

==> tables/results_2DHydro.tex <==
\scriptsize
\centering
\begin{tabular}{llrrll}
\toprule\bfseries \# uniform ref & \bfseries \#-elem & \bfseries \# nodes. & \bfseries err$_m$ \\\midrule
1 & 272.    & 159       & 0.000512563\\
2 & 1088   & 589      & 8.50172e-05\\
3 & 4352   & 2265     & 1.66138e-05\\
4 & 17408  &  8881   &  4.06608e-06\\
5 & 69632  & 35169   & 1.92418e-06\\
6 & 278528 & 139969 &1.30185e-06\\
\bottomrule
\end{tabular}

\vspace{1cm}



==> tables/table_methods.tex <==
\scriptsize
\centering
\begin{tabular}{llrrllll}
\toprule\bfseries Method & \bfseries \#-matr. & \bfseries \#-frac. & \bfseries d.o.f. & \bfseries err$_m$ & \bfseries err$_f$ & \bfseries nnz/size$^2$ & \bfseries $\| \cdot \|_2$-cond.\\\midrule
Embedded equi-dimension model$^2$ & 1496 quads & 78 & 1733.0 & 1.2e-2 & 7.6e-3 & 5.2e-3 & 5.4e12\\
Embedded hybrid-dimensional model$^2$ - dual-Lagr.-Mult. & 1496 quads & 78 & 1575.0 & 1.2e-2 & 7.6e-3 & 6.6e-3 & 7.9e10\\
Mortar equi-dimesional model$^2$ - p0-Lagr.-Mult. & 1496 quads & 78 & 1732.0 & 1.2e-2 & 7.8e-3 & 5.0e-3 & 2.8e12\\
\bottomrule
\end{tabular}
